Error-feedback stochastic modeling strategy for time series forecasting with convolutional neural networks

Despite the superiority of convolutional neural networks demonstrated in time series modeling and forecasting, it has not been fully explored on the design of the neural network architecture and the tuning of the hyper-parameters. Inspired by the incremental construction strategy for building a random multilayer perceptron, we propose a novel Error-feedback Stochastic Modeling (ESM) strategy to construct a random Convolutional Neural Network (ESM-CNN) for time series forecasting task, which builds the network architecture adaptively. The ESM strategy suggests that random filters and neurons of the error-feedback fully connected layer are incrementally added to steadily compensate the prediction error during the construction process, and then a filter selection strategy is introduced to enable ESM-CNN to extract the different size of temporal features, providing helpful information at each iterative process for the prediction. The performance of ESM-CNN is justified on its prediction accuracy of one-step-ahead and multi-step-ahead forecasting tasks respectively. Comprehensive experiments on both the synthetic and real-world datasets show that the proposed ESM-CNN not only outperforms the state-of-art random neural networks, but also exhibits stronger predictive power and less computing overhead in comparison to trained state-of-art deep neural network models.

==> tables/ar1.tex <==
\begin{sidewaystable*}[!htp]
	\centering
	\footnotesize
	\caption{The average performance of ESM-CNN and the counterparts on AR1 dataset. \label{tab:results_ar1}}
	\begin{tabularx}{\textwidth}{ccYYYYYYYYY}
		\toprule
		\multirow{2}{*}{Measure} & \multirow{2}{*}{$H$} & \multicolumn{3}{c}{Training based counterparts} & \multicolumn{3}{c}{Random based counterparts} & \multicolumn{2}{c}{Ablative based counterparts} & Our                                                                                                                                     \\ 
		\cmidrule(l){3-5} \cmidrule(l){6-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
		                      &   & GS-CNN          & DeepAR          & CLSTM           & RVFL              & IELM            & SCN             & Stoc-CNN            & ES-CNN                  & ESM-CNN                         \\
		\midrule
		\multirowcell{6}{MAPE                                                                                                                                                                                                     \\ $(\%)$}    & 1 & 8.753 (0.0055)  & 10.831 (0.0226) & 8.885 (0.0142)  & 76.091 (0.4745)   & 9.838 (0.0147)  & 6.504 (0.0241)  & 6096.954 (25.1571)  & \textbf{4.527 (0.0058)} & \textbf{3.485$^\star$ (0.0005)} \\

		                      & 3 & 10.851 (0.0067) & 16.440 (0.0346) & 12.021 (0.0134) & 116.972 (0.5849)  & 10.660 (0.0122) & 9.532 (0.0197)  & 6340.421 (21.2825)  & \textbf{6.415 (0.0052)} & \textbf{5.277$^\star$ (0.0018)} \\

		                      & 6 & 13.314 (0.0070) & 21.654 (0.0372) & 12.404 (0.0184) & 123.468 (0.7779)  & 12.642 (0.0174) & 11.566 (0.0263) & 15395.348 (80.1823) & \textbf{8.924 (0.0052)} & \textbf{7.695$^\star$ (0.0023)} \\

		\multirowcell{6}{SMAPE                                                                                                                                                                                                    \\ $(\%)$}   & 1 & 4.657 (0.0032)  & 5.807 (0.0128)  & 4.739 (0.0084)  & 301.885 (6.7403)  & 5.302 (0.0088)  & 3.400 (0.0135)  & 121.230 (0.5129)    & \textbf{2.330 (0.0032)} & \textbf{1.760$^\star$ (0.0003)} \\

		                      & 3 & 5.884 (0.0039)  & 9.173 (0.0210)  & 6.611 (0.0082)  & 860.693 (10.7220) & 5.761 (0.0074)  & 5.110 (0.0115)  & 150.318 (1.3617)    & \textbf{3.356 (0.0029)} & \textbf{2.718$^\star$ (0.0010)} \\

		                      & 6 & 7.372 (0.0042)  & 12.482 (0.0241) & 6.816 (0.0117)  & 635.775 (6.5927)  & 6.974 (0.0106)  & 6.281 (0.0162)  & 152.014 (1.7270)    & \textbf{4.777 (0.0030)} & \textbf{4.053$^\star$ (0.0015)} \\

		\multirow{6}{*}{RMSE} & 1 & 0.462 (0.0311)  & 0.508 (0.0960)  & 0.489 (0.0893)  & 3.211 (1.8512)    & 0.554 (0.0781)  & 0.334 (0.1134)  & 436.078 (201.3846)  & \textbf{0.228 (0.0343)} & \textbf{0.155$^\star$ (0.0037)} \\
		                      & 3 & 0.567 (0.0337)  & 0.766 (0.1305)  & 0.667 (0.0671)  & 5.152 (2.2614)    & 0.580 (0.0650)  & 0.498 (0.0872)  & 443.439 (194.6141)  & \textbf{0.322 (0.0243)} & \textbf{0.257$^\star$ (0.0104)} \\

		                      & 6 & 0.683 (0.0300)  & 0.996 (0.1339)  & 0.679 (0.0910)  & 5.591 (3.2707)    & 0.671 (0.0789)  & 0.600 (0.1270)  & 1065.447 (536.6946) & \textbf{0.461 (0.0271)} & \textbf{0.394$^\star$ (0.0162)} \\
		\bottomrule
	\end{tabularx}
\end{sidewaystable*}

==> tables/gold.tex <==
\begin{sidewaystable*}[!ht]
    \centering
    \footnotesize
    \caption{The average performance of ESM-CNN and the counterparts on GOLD dataset. \label{tab:results_gold}}
    \begin{tabularx}{\textwidth}{ccYYYYYYYYY}
        \toprule
        \multirow{2}{*}{Measure} & \multirow{2}{*}{$H$} & \multicolumn{3}{c}{Training based counterparts} & \multicolumn{3}{c}{Random based counterparts} & \multicolumn{2}{c}{Ablative based counterparts} & Our                                                                                                                        \\ \cmidrule(l){3-5} \cmidrule(l){6-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
                                 &                      & GS-CNN                                          & DeepAR                                        & CLSTM                                           & RVFL            & IELM            & SCN                     & Stoc-CNN        & ES-CNN          & ESM-CNN                  \\
        \midrule
        \multirow{6}{*}{mape}    & 1                    & 0.674 (0.0000)                                  & 0.551 (0.0002)                                & 0.566 (0.0002)                                  & 0.562 (0.0001)  & 0.988 (0.0012)  & \textbf{0.541 (0.0001)}          & 4.018 (0.0057)  & 0.564 (0.0002)  & \textbf{0.538$^\star$ (0.0000)}  \\
                                 & 5                    & 0.980 (0.0000)                                  & 1.001 (0.0007)                                & 1.022 (0.0009)                                  & 0.902 (0.0003)  & 1.280 (0.0028)  & \textbf{0.867 (0.0002)}          & 4.608 (0.0033)  & 0.885 (0.0000)  & \textbf{0.864$^\star$ (0.0001)}  \\
                                 & 10                   & 1.311 (0.0002)                                  & 1.359 (0.0008)                                & 1.402 (0.0009)                                  & 1.246 (0.0003)  & 1.745 (0.0053)  & \textbf{1.200$^\star$ (0.0002)}          & 4.879 (0.0021)  & 1.224 (0.0001)  & \textbf{1.202 (0.0000)}  \\
        \multirow{6}{*}{smape}   & 1                    & 0.337 (0.0000)                                  & 0.276 (0.0001)                                & 0.283 (0.0001)                                  & 0.281 (0.0001)  & 0.495 (0.0006)  & \textbf{0.271 (0.0000)}          & 1.988 (0.0027)  & 0.282 (0.0001)  & \textbf{0.269$^\star$ (0.0000)}  \\
                                 & 5                    & 0.492 (0.0000)                                  & 0.503 (0.0003)                                & 0.514 (0.0004)                                  & 0.452 (0.0001)  & 0.642 (0.0014)  & \textbf{0.435 (0.0001)}          & 2.313 (0.0017)  & 0.444 (0.0000)  & \textbf{0.433$^\star$ (0.0000)}  \\
                                 & 10                   & 0.659 (0.0001)                                  & 0.685 (0.0004)                                & 0.706 (0.0005)                                  & 0.627 (0.0002)  & 0.880 (0.0028)  & \textbf{0.602$^\star$ (0.0001)} & 2.467 (0.0011)  & 0.615 (0.0001)  & \textbf{0.604 (0.0000)}         \\
        \multirow{6}{*}{rmse}    & 1                    & 11.194 (0.0637)                                 & 9.115 (0.2177)                                & 9.200 (0.2096)                                  & 9.248 (0.2067)  & 15.775 (1.9461) & \textbf{8.927 (0.0926)}          & 67.726 (8.6392) & 9.305 (0.4227)  & \textbf{8.812$^\star$ (0.0523)}  \\
                                 & 5                    & 16.088 (0.0793)                                 & 17.119 (1.1618)                               & 16.845 (1.3806)                                 & 15.232 (0.3726) & 20.351 (4.1984) & \textbf{14.630 (0.2255)}         & 78.742 (5.5579) & 14.786 (0.0556) & \textbf{14.491$^\star$ (0.0650)} \\
                                 & 10                   & 21.215 (0.3222)                                 & 22.968 (1.2059)                               & 22.680 (1.2820)                                 & 21.227 (0.5558) & 27.452 (7.7176) & \textbf{19.924 (0.2044)}         & 84.875 (3.9404) & 20.216 (0.2090) & \textbf{19.877$^\star$ (0.0653)}
        \\
        \bottomrule
    \end{tabularx}
\end{sidewaystable*}

==> tables/ili.tex <==
\begin{sidewaystable*}[!htp]
    \centering
    \footnotesize
    \caption{The average performance of ESM-CNN and the counterparts on ILI dataset. \label{tab:results_ili}}
    \begin{tabularx}{\textwidth}{ccYYYYYYYYY}
        \toprule
        \multirow{2}{*}{Measure} & \multirow{2}{*}{$H$} & \multicolumn{3}{c}{Training based counterparts} & \multicolumn{3}{c}{Random based counterparts} & \multicolumn{2}{c}{Ablative based counterparts} & Our                                                                                                                                 \\ \cmidrule(l){3-5} \cmidrule(l){6-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
                                 &                      & GS-CNN                                          & DeepAR                                        & CLSTM                                           & RVFL            & IELM            & SCN             & Stoc-CNN         & ES-CNN                  & ESM-CNN                          \\
        \midrule
        \multirowcell{6}{MAPE                                                                                                                                                                                                                                                                                                                     \\ $(\%)$}    & 1 & 10.787 (0.0018) & 11.448 (0.0089) & \textbf{9.499 (0.0026)}  & 30.302 (0.0517) & 13.781 (0.0081) & 11.483 (0.0095) & 248.333 (0.3722) & 10.007 (0.0096)         & \textbf{8.927$^\star$ (0.0031)}  \\
                                 & 4 & 13.562 (0.0018) & 15.883 (0.0075) & \textbf{12.600 (0.0019)} & 35.281 (0.0388) & 15.799 (0.0054) & 15.322 (0.0090) & 232.743 (0.2252) & 13.304 (0.0046)         & \textbf{12.523$^\star$ (0.0039)} \\
                                 & 8 & 15.885 (0.0029) & 18.237 (0.0087) & \textbf{14.482$^\star$ (0.0032)} & 36.668 (0.0419) & 17.417 (0.0048) & 18.564 (0.0111) & 238.353 (0.3148) & 16.206 (0.0041)         & \textbf{15.309 (0.0033)} \\
        \multirowcell{6}{SMAPE                                                                                                                                                                                                                                                                                                                    \\ $(\%)$}   & 1 & 5.746 (0.0010)  & 6.025 (0.0044)  & \textbf{4.863 (0.0015)}  & 12.826 (0.0173) & 7.489 (0.0047)  & 6.064 (0.0051)  & 96.461 (0.5607)  & 5.200 (0.0051)          & \textbf{4.598$^\star$ (0.0014)}  \\
                                 & 4 & 7.387 (0.0010)  & 8.431 (0.0033)  & \textbf{6.713 (0.0011)}  & 16.386 (0.0167) & 8.827 (0.0036)  & 8.240 (0.0050)  & 138.547 (0.4767) & 7.128 (0.0024)          & \textbf{6.645$^\star$ (0.0020)}  \\
                                 & 8 & 9.013 (0.0017)  & 10.005 (0.0037) & \textbf{8.107$^\star$ (0.0020)}  & 25.549 (0.1625) & 10.067 (0.0032) & 10.421 (0.0064) & 159.782 (0.5971) & 9.065 (0.0022)          & \textbf{8.519 (0.0018)}  \\

        \multirow{6}{*}{RMSE}    & 1 & 0.748 (0.0095)  & 0.782 (0.0187)  & 0.710 (0.0252)           & 1.738 (0.3170)  & 0.888 (0.0441)  & 0.714 (0.0311)  & 15.049 (2.4962)  & \textbf{0.681 (0.0537)} & \textbf{0.606$^\star$ (0.0081)}  \\

                                 & 4 & 0.909 (0.0063)  & 0.995 (0.0152)  & 0.907 (0.0171)           & 1.962 (0.2486)  & 1.038 (0.0356)  & 0.909 (0.0252)  & 13.880 (1.5402)  & \textbf{0.865 (0.0235)} & \textbf{0.814$^\star$ (0.0087)}  \\

                                 & 8 & 1.085 (0.0072)  & 1.156 (0.0211)  & \textbf{1.040 (0.0176)}  & 2.000 (0.2323)  & 1.179 (0.0207)  & 1.112 (0.0254)  & 14.254 (2.0343)  & 1.067 (0.0107)          & \textbf{1.030$^\star$ (0.0066)} \\
        \bottomrule
    \end{tabularx}
\end{sidewaystable*}

==> tables/time_trans.tex <==
\begin{table*}[!h]
    \centering
    \footnotesize
    \caption{The average running time (seconds) of each model on both two datasets. \label{tab:time}}
    \begin{tabularx}{\textwidth}{ccYYYYYY}
        \toprule
        \multirow{2}{*}{Methods}   & \multirow{2}{*}{Models} & \multicolumn{3}{c}{AR1} & \multicolumn{3}{c}{ILI}                                           \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8}
                                   &                         & 1                       & 3                       & 6      & 1        & 4        & 8        \\
        \midrule
        \multirowcell{3}{Training} & GS-CNN                  & 228.00                  & 230.40                  & 232.25 & 239.35   & 190.80   & 192.60   \\
                                   & DeepAR                  & 225.25                  & 238.95                  & 257.70 & 256.80   & 279.10   & 275.30   \\
                                   & CLSTM                   & 150.45                  & 154.80                  & 160.25 & 167.40   & 170.80   & 175.30   \\
        \specialrule{0em}{1.5pt}{1.5pt}
        \multirowcell{3}{Random }  & RVFL                    & -                       & -                       & -      & -        & -        & -        \\
                                   & IELM                    & \ph\ph2.65                    & \ph\ph2.85                    & \ph\ph2.80   & \ph\ph2.55     & \ph\ph2.55     & \ph\ph2.40     \\
                                   & SCN                     & \ph22.85                & \ph57.40                & 107.75 & \ph16.10 & \ph49.60 & \ph90.95 \\
        \specialrule{0em}{1.5pt}{1.5pt}
        \multirowcell{2}{Ablation} & Stoc-CNN                & -                       & -                       & -      & -        & -        & -        \\
                                   & ES-CNN                  & \ph\ph6.50                    & \ph\ph6.40                    & \ph\ph6.50   & \ph\ph6.45     & \ph\ph6.50     & \ph\ph6.50     \\
        \specialrule{0em}{1.5pt}{1.5pt}
        Our                        & ESM-CNN                 & \ph\ph9.65                    & \ph\ph9.65                    & \ph\ph9.70   & \ph\ph7.15     & \ph\ph7.15     & \ph\ph7.20     \\
        \bottomrule
    \end{tabularx}
\end{table*}
